A bio-inspired implementation of a sparse-learning spike-based hippocampus memory model

The nervous system, more specifically, the brain, is capable of solving complex problems simply and efficiently, far surpassing modern computers. In this regard, neuromorphic engineering is a research field that focuses on mimicking the basic principles that govern the brain in order to develop systems that achieve such computational capabilities. Within this field, bio-inspired learning and memory systems are still a challenge to be solved, and this is where the hippocampus is involved. It is the region of the brain that acts as a short-term memory, allowing the learning and unstructured and rapid storage of information from all the sensory nuclei of the cerebral cortex and its subsequent recall. In this work, we propose a novel bio-inspired memory model based on the hippocampus with the ability to learn memories, recall them from a cue (a part of the memory associated with the rest of the content) and even forget memories when trying to learn others with the same cue. This model has been implemented on the SpiNNaker hardware platform using Spiking Neural Networks, and a set of experiments and tests were performed to demonstrate its correct and expected operation. The proposed spike-based memory model generates spikes only when it receives an input, being energy efficient, and it needs 7 timesteps for the learning step and 6 timesteps for recalling a previously-stored memory. This work presents the first hardware implementation of a fully functional bio-inspired spike-based hippocampus memory model, paving the road for the development of future more complex neuromorphic systems.

==> doc/estructura.tex <==

Abstract
    - Introduction
        - Biological model of the hippocampus
        - Related works
        - Main contribution
    - Materials and methods
        - SNN
        - Spinnaker
    - Sparse-learning hippocampus computational memory model
        - Architecture
            - DG
            - CA3
            - CA1
            - Connections
        - Operating principle
            - Input and output
            - Implemented functionality
        - Resources and timing constraints
    - Experimentation and results
        - Learning
        - Learning and recall
        - Learning, forgetting and relearning
        - Combined operations sequence test
        - Random learning and recall test
        - Stress memory testbench
    - Discussion
        - Comparison with state-of-the-art works
        - Limitations
    - Conclusions
Bibliography




Introduction:
        - Importancia de las tecnologías neuromórficas y bioinspiradas (enfocando la explicación a sistemas de aprendizaje)
	    - Las redes neuronales pulsantes (SNN) o redes neuronales de tercera generación
	    - El hipocampo y sus funciones como memoria a corto plazo
	    - Modelos computacionales de memoria a corto plazo inspiradas en el hipocampo en el estado del arte
	    - Hablar de la falta de modelos funcionales en casos reales de uso de esta tecnología y la propuesta de 2 nuevos modelos, ambos bioinspirados pero uno con un enfoque más biológico y otro más funcional
	    - Contribuciones

    + Biological model of the hippocampus
        - Sistema límbico
        - Explicar en profundidad las diferentes partes del hipocampo
        - Funcionalidad
    
    + Related works
        - Estado del arte extendido
        - CA3 memory model with oscillatory activity
        - CA3 memory model with regulated periods of activity
    
    + Main contribution
        - Extenderse con las contribuciones


Materials and methods
    + SNN
        - Hablar sobre neuronas, sinapsis, stdp, ... en detalle (mirar TFM), y los parámetros


Sparse-learning hippocampus computational memory model
        - A nivel de bloque comentar las entradas y salidas, funcionamiento general, arquitectura de la memoria y simil con modelo biológico
    + Architecture
        + DG
        + CA3
        + CA1
        + Connections
    + Operation principles
        + Input and output
        + Implemented functionality
            - Learning, recall and forgetting and relearning -> como funcionan internamente en la red
            - Detallar el timing interno de la red, por cada capa, y de las operaciones (mirar word)
    + Resources and timing constraints
        - Tabla resumen de los recursos necesarios y los tiempos de operaciones más a nivel de usuario (sin detalles internos de la red, eso va en el apartado de operaciones)


Experimentation and results


Discussion
    + Comparison with state-of-the-art works
        - Comparar en todos los apartados que se pueda: recursos, funcional, temporización, ..., no solo con los nuestros modelos anteriores, sino también con los demás del estado del arte


Conclusions


==> doc/formatos.tex <==

% Figura normal
\begin{figure}[!t]
\centering
\includegraphics[width=2.5in]{fig1}
\caption{Simulation results for the network.}
\label{fig_1}
\end{figure}

% 2 figuras con ancho completo
\begin{figure*}[!t]
\centering
\subfloat[]{\includegraphics[width=2.5in]{fig1}%
\label{fig_first_case}}
\hfil
\subfloat[]{\includegraphics[width=2.5in]{fig1}%
\label{fig_second_case}}
\caption{Dae. Ad quatur autat ut porepel itemoles dolor autem fuga. Bus quia con nessunti as remo di quatus non perum que nimus. (a) Case I. (b) Case II.}
\label{fig_sim}
\end{figure*}

==> sections/acknowledgments.tex <==
\section*{Acknowledgments}
This research was partially supported by the Spanish grant MINDROB (PID2019-105556GB-C33/AEI/10.13039/501100011033). D. C.-M. was supported by a "Formaci\'{o}n de Profesor Universitario" Scholarship from the Spanish Ministry of Education, Culture and Sport.
